Seeing Stereotypes

Reliance on stereotypes is a persistent feature of human decision-making and has been extensively documented in educational settings, where it can shape students' confidence, performance, and long-term human capital accumulation. While effective techniques exist to mitigate these negative effects, a crucial first step is to establish whether teachers can recognize stereotypes in their professional environment. We introduce the Stereotype Identification Test (SIT), a novel survey tool that asks teachers to evaluate and comment on the presence of stereotypes in images randomly drawn from school textbooks. Their responses are systematically linked to established measures of implicit bias (Implicit Association Test, IAT) and explicit bias (survey scales on teaching stereotypes and social values). Our findings demonstrate that the SIT is a valid and reliable measure of stereotype recognition. Teachers' ability to recognize stereotypes is linked to trainable traits such as implicit bias awareness and inclusive teaching practices. Moreover, providing personalized feedback on implicit bias improves SIT scores by 0.25 standard deviations, reinforcing the idea that stereotype recognition is malleable and can be enhanced through targeted interventions.

==> tables/First_Framing.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Framing and IAT first on SIT}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
SIT first + Info&       0.116         &       0.104         &       0.191\sym{*}  \\
            &     (0.106)         &     (0.104)         &    (0.0993)         \\
[1em]
SIT first + No framing&     0.00229         &     0.00184         &      0.0896         \\
            &     (0.100)         &    (0.0980)         &    (0.0959)         \\
[1em]
IAT first + Info + Guilt&       0.367\sym{***}&       0.342\sym{***}&       0.339\sym{***}\\
            &     (0.128)         &     (0.123)         &     (0.109)         \\
[1em]
IAT first + Info &       0.277\sym{**} &       0.250\sym{**} &       0.253\sym{**} \\
            &     (0.126)         &     (0.124)         &     (0.112)         \\
[1em]
IAT first + No framing&       0.203         &       0.199         &       0.235\sym{**} \\
            &     (0.134)         &     (0.133)         &     (0.119)         \\
[1em]
IAT Score   &                     &                     &       0.126\sym{*}  \\
            &                     &                     &    (0.0741)         \\
[1em]
Growth Mind &                     &                     &      0.0122         \\
            &                     &                     &    (0.0372)         \\
[1em]
Implicit Bias Awareness&                     &                     &       0.256\sym{***}\\
            &                     &                     &    (0.0476)         \\
[1em]
Gender Stem &                     &                     &     -0.0374         \\
            &                     &                     &    (0.0378)         \\
[1em]
Locus of Control&                     &                     &      0.0929\sym{**} \\
            &                     &                     &    (0.0455)         \\
[1em]
Social Values&                     &                     &       0.137\sym{***}\\
            &                     &                     &    (0.0466)         \\
[1em]
Inclusive Teaching&                     &                     &      0.0848\sym{*}  \\
            &                     &                     &    (0.0436)         \\
[1em]
Gender     &                     &       0.270\sym{**} &      0.0835         \\
            &                     &     (0.105)         &    (0.0980)         \\
[1em]
Age         &                     &      0.0107\sym{***}&      0.0107\sym{***}\\
            &                     &   (0.00356)         &   (0.00334)         \\
[1em]
Like Teach  &                     &     -0.0490         &     -0.0910\sym{***}\\
            &                     &    (0.0339)         &    (0.0311)         \\
[1em]
\hline\hline
\end{tabular}
\end{table}

\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption*{Framing on SIT - Cont}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
Master      &                     &      0.0448         &      0.0485         \\
            &                     &    (0.0882)         &    (0.0806)         \\
[1em]
LD Training &                     &       0.131         &      0.0171         \\
            &                     &    (0.0797)         &    (0.0740)         \\
[1em]
Married     &                     &     -0.0235         &     -0.0448         \\
            &                     &    (0.0743)         &    (0.0695)         \\
[1em]
Teaching Italian&                     &      0.0935         &    -0.00316         \\
            &                     &    (0.0746)         &    (0.0698)         \\
[1em]
Teaching Maths&                     &       0.126         &       0.172\sym{*}  \\
            &                     &    (0.0929)         &    (0.0890)         \\
[1em]
Lexical Density &                     &                     &       0.507\sym{**} \\
            &                     &                     &     (0.245)         \\
[1em]
Lexical Variety     &                     &                     &       0.197         \\
            &                     &                     &     (0.327)         \\
[1em]
\_cons      &      -0.116         &      -0.694\sym{**} &      -0.700\sym{**} \\
            &    (0.0715)         &     (0.275)         &     (0.346)         \\
[1em]
\hline
\(N\)       &         627         &         627         &         621         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Dependent variable: SIT Score}\\
\multicolumn{4}{l}{\footnotesize Omitted category in framing: SIT first + Info + Guilt}\\
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> tables/Framing_test.tex <==

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\begin{longtable}{l*{3}{c}}
\caption{Framing on SIT} 
\label{tab:framing} \\
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
\endfirsthead

\hline\hline
\caption*{(Continued) Framing on SIT} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
\endhead

\hline
\multicolumn{4}{r}{\footnotesize Continues in the next page} \\
\endfoot

\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses} \\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)} \\
\endlastfoot

Info                &       0.065         &       0.035         &       0.091         \\
                    &     (0.099)         &     (0.097)         &     (0.089)         \\
[1em]
No framing          &      -0.051         &      -0.054         &      -0.001         \\
                    &     (0.098)         &     (0.096)         &     (0.089)         \\
[1em]
IAT Revelation      &                     &       0.276\sym{***}&       0.217\sym{***}\\
                    &                     &     (0.085)         &     (0.076)         \\
[1em]
Gender              &                     &       0.305\sym{**} &       0.127         \\
                    &                     &     (0.122)         &     (0.115)         \\
[1em]
Age                 &                     &       0.013\sym{***}&       0.012\sym{***}\\
                    &                     &     (0.004)         &     (0.004)         \\
[1em]
Like Teaching       &                     &      -0.057         &      -0.122\sym{***}\\
                    &                     &     (0.042)         &     (0.037)         \\
[1em]
Master              &                     &       0.057         &       0.039         \\
                    &                     &     (0.105)         &     (0.096)         \\
[1em]
Disability training &                     &       0.124         &       0.013         \\
                    &                     &     (0.093)         &     (0.086)         \\
[1em]
Married             &                     &      -0.028         &      -0.067         \\
                    &                     &     (0.086)         &     (0.080)         \\
[1em]
Teaching Italian    &                     &       0.073         &      -0.005         \\
                    &                     &     (0.086)         &     (0.081)         \\
[1em]
Teaching Maths      &                     &       0.149         &       0.216\sym{**} \\
                    &                     &     (0.108)         &     (0.103)         \\
[1em]
Isole               &                     &      -0.032         &      -0.139         \\
                    &                     &     (0.160)         &     (0.147)         \\
[1em]
Missing             &                     &      -0.096         &      -0.080         \\
                    &                     &     (0.191)         &     (0.165)         \\
[1em]
Nord-Est            &                     &      -0.046         &      -0.098         \\
                    &                     &     (0.142)         &     (0.129)         \\
[1em]
Nord-Ovest          &                     &      -0.102         &      -0.118         \\
                    &                     &     (0.128)         &     (0.119)         \\
[1em]
Sud                 &                     &      -0.204         &      -0.269\sym{**} \\
                    &                     &     (0.141)         &     (0.133)         \\
[1em]
IAT score           &                     &                     &       0.049         \\
                    &                     &                     &     (0.042)         \\
[1em]
Growth Mindset      &                     &                     &       0.036         \\
                    &                     &                     &     (0.043)         \\
[1em]
Implicit Bias Awareness&                     &                     &       0.266\sym{***}\\
                    &                     &                     &     (0.053)         \\
[1em]
Gender-STEM Stereotypes&                     &                     &      -0.042         \\
                    &                     &                     &     (0.043)         \\
[1em]
Locus of Control    &                     &                     &       0.108\sym{**} \\
                    &                     &                     &     (0.053)         \\
[1em]
Social Values       &                     &                     &       0.148\sym{***}\\
                    &                     &                     &     (0.053)         \\
[1em]
Inclusive Teaching  &                     &                     &       0.107\sym{**} \\
                    &                     &                     &     (0.050)         \\
[1em]
Lexical Density     &                     &                     &       0.671\sym{***}\\
                    &                     &                     &     (0.236)         \\
[1em]
Constant            &      -0.004         &      -0.667\sym{*}  &      -0.335         \\
                    &     (0.069)         &     (0.366)         &     (0.360)         \\
\hline
Observations        &         614         &         614         &         614         \\
\end{longtable}



